A Survey of LLM $\times$ DATA

The integration of large language model (LLM) and data management (DATA) is rapidly redefining both domains. In this survey, we comprehensively review the bidirectional relationships. On the one hand, DATA4LLM, spanning large-scale data processing, storage, and serving, feeds LLMs with high quality, diversity, and timeliness of data required for stages like pre-training, post-training, retrieval-augmented generation, and agentic workflows: (i) Data processing for LLMs includes scalable acquisition, deduplication, filtering, selection, domain mixing, and synthetic augmentation; (ii) Data Storage for LLMs focuses on efficient data and model formats, distributed and heterogeneous storage hierarchies, KV-cache management, and fault-tolerant checkpointing; (iii) Data serving for LLMs tackles challenges in RAG (e.g., knowledge post-processing), LLM inference (e.g., prompt compression, data provenance), and training strategies (e.g., data packing and shuffling). On the other hand, in LLM4DATA, LLMs are emerging as general-purpose engines for data management. We review recent advances in (i) data manipulation, including automatic data cleaning, integration, discovery; (ii) data analysis, covering reasoning over structured, semi-structured, and unstructured data, and (iii) system optimization (e.g., configuration tuning, query rewriting, anomaly diagnosis), powered by LLM techniques like retrieval-augmented prompting, task-specialized fine-tuning, and multi-agent collaboration.

==> response/Summary.tex <==
%!TEX root = ../main.tex


%\vspace{-.5em}
%\subsection*{Summary of the Revision}
%\vspace{-.25em}
%\vspace{.5em}



==> response/general.tex <==
%!TEX root = ../main.tex

\subsection*{Dear Reviewers,}

Thank you for your thoughtful reviews and encouraging comments in the second-round review. We have significantly improved the paper based on your valuable comments. The revised parts are highlighted in \overwrite{blue} and the responses are summarized below.

==> response/meta.tex <==
%!TEX root = ../main.tex

% ....

\vspace{-.5em}
\subsection*{Responses to the Associate Editor}

%\vspace{-1.em}

%\mybox{
%\stitle{Summary Comment:}
%{\em The reviewers show support to this work, and request revision to further address their concerns. Please refer to the reviewers' comments for details.} 

\begin{Box4}{}
	{\underline{\textit{COMMENT}}: R3 further give a lot of constructive and detailed suggestions for improving the paper, mentioning problems such as unrealistic claims, improper title, missing citations, etc. Therefore, another round of revision is needed for this survey.  .} 
\end{Box4}

\stitle{\bfit{Response:}} We thank the associate editor for the coordination of our survey. Based on the new comments of the reviewers, we have significantly improved the paper and addressed all the comments. We summarize the changes as follows. 
\vspace{.5em}

\stitle{\underline{\bfit{Title:}}}  We have changed  the title to ``Automatic Database Knob Tuning: A Survey'' and made it consistent throughout the paper (see R3C1).
\vspace{.5em}
 
\stitle{\underline{\bfit{Section 1 \& Section 2 (Intro \& Framework):}}} 
First, we have added the four aspects of tuning evaluation in Section~\ref{sec:introducion} (see R3C3). Second, we have clarified the definition of configuration space in knob tuning (Section~\ref{subsec:challenge}). Third, we have updated the description of BO-based and RL-based tuning methods in Section~\ref{sec:framework} (see R3C2).

\vspace{.5em}
\stitle{\underline{\bfit{Section 3 (Knob Selection):}}} First, we have added the discussion of categorical knobs in Definition 1 (Section~\ref{subsec:knobs}). Second, we have added more details of configuration knobs, including $(i)$ the insights of the knob effects and $(ii)$ concrete knob examples in Section~\ref{subsec:process} (see R3C8, R3C11). Besides, we have removed the category of {\it learning-based knob selection} (see R3C4).

%Third, we have updated Figure~\ref{fig:knobs} to make it consistent with Section~\ref{subsec:knobs}.  

\vspace{.5em}
\stitle{\underline{\bfit{Section 4 (Feature Selection):}}}  \lgl{???? -added} 
We have reorganized this section and clarified the relations between tuning objective metrics and knobs (see R3C5).



\vspace{.5em}
\stitle{\underline{\bfit{Section 5 (Tuning Methods):}}} %We have reorganized the Section~\ref{subsec:gp} (R3C2, R3C6). 
First, we have renamed GP-based tuning methods into BO-based tuning methods. Second, we have separately introduced the common modules in BO-based tuning methods, \ie the surrogate model, acquisition functions, model initialization, and database features (see R3C2, R3C6). Third, for each subsection, we have added a remark to summarize the pros and cons of the corresponding tuning methods based on the experimental researches~\cite{van2021inquiry,DBLP:journals/pvldb/ZhangCLWTLC22} (see R3C10).


%\vspace{.5em}
%\stitle{\underline{\bfit{Section 6 \& Section 7 (Tuning Deployment \& Challenges):}}}  We have carefully proofread the whole paper and fixed all the errors.



==> response/r1.tex <==
%!TEX root = ../main.tex

\vspace{-.5em}
\subsection*{Responses to Reviewer \#1}

\begin{Box4}{}
	{\textbf{C1}: Go through the paper and fix the obvious errors.} 
\end{Box4} 

\stitle{\bfit{Response:}}  We have carefully proofread the whole paper and fixed all the errors.

\iffalse

Section~\ref{subsec:contributions}: ``transferring techniques'' $\rightarrow$ ``transfer techniques'';

%Section~\ref{subsec:access}: ``Thus it is challenging ...'' $\rightarrow$ ``Thus, it is challenging ...'';

Section~\ref{subsec:computation}: ``\eg {\it max\_file ...}'' $\rightarrow$ ``\eg\ {\it max\_file ...}'';
\vspace{.25em}

%Section~\ref{subsec:ks}: ``...have major impact on ...'' $\rightarrow$ ``have a major impact on'';

%Section~\ref{subsec:drl}: ``QTune used ...'' $\rightarrow$ ``QTune uses ...'';

Section~\ref{subsec:metric selection}: ``... metrics in database'' $\rightarrow$ ``... metrics in the database'';
\vspace{.25em}

Section~\ref{subsec:heuristic}: ``the quality of each search methodand ...'' $\rightarrow$ ``the quality of each search method and ...''; %``... Although the search-based tuning method can not guarantee ...'' $\rightarrow$ ``Although the search-based tuning method cannot guarantee ...''
\vspace{.25em}

Section~\ref{subsec:drl}: ``QTune used a modified DDPG model ...'' $\rightarrow$ ``QTune uses a modified DDPG model ...'';
\vspace{.25em}

%Section~\ref{subsec:drl}: ``RL-based tuning model, UDO [81],HUNTER [9], and DB-BERT [76] are proposed ...'' $\rightarrow$ ``RL-based tuning model, UDO [81], HUNTER [9], and DB-BERT [76] are proposed ...'';

Table~\ref{tbl:methodsummary}: ``Esemble'' $\rightarrow$ ``Ensemble'';
\vspace{.25em}

Section~\ref{subsec:rdbms}: ``accumated'' $\rightarrow$ ``accumulated'';
\vspace{.25em}

\fi


==> response/r2.tex <==
%!TEX root = ../main.tex

\vspace{-.5em}
\subsection*{Responses to Reviewer \#2}

%\vspace{-.5em}

\begin{Box4}{}
	{\textbf{C1}: This revised paper well addressed the issues raised by the reviewers. It could be better to mention some missing related works as follows which also surveyed the database configuration and knob tuning:\\
		(1) Herodotos Herodotou, Yuxing Chen, Jiaheng Lu: A Survey on Automatic Parameter Tuning for Big Data Processing Systems. ACM Comput. Surv. 53(2): 43:1-43:37 (2020)
		\\
		(2) Jiaheng Lu, Yuxing Chen, Herodotos Herodotou, Shivnath Babu:
		Speedup Your Analytics: Automatic Parameter Tuning for Databases and Big Data Systems. Proc. VLDB Endow. 12(12): 1970-1973 (2019)
	}
\end{Box4}

%\vspace{-.6em}
\stitle{\bfit{Response:}} We have added these two references~\cite{herodotou2020survey,DBLP:journals/pvldb/LuCHB19} in Section~\ref{sec:introducion} and Section~\ref{subsec:bigdata}. 
%These works studied many classic knob tuning methods (\eg cost-based approaches, empirical approaches, ML approaches). However,  \cite{herodotou2020survey} mainly focuses on big data systems, and \cite{DBLP:journals/pvldb/LuCHB19} is a great tutorial paper. Instead, in this paper, we aim to thoroughly and extensively survey the knob tuning methods for databases, and provide a finer-grained analysis (\ie\ feature selection, knob selection, tuning methodologies, and transfer techniques).


==> response/r3.tex <==
%!TEX root = ../main.tex
 
\vspace{-.5em}
\subsection*{Responses to Reviewer \#3}

%\vspace{-1.em}

\begin{Box4}{}
	{\textbf{C1}: As a survey paper titled “Automatic Database Configuration Tuning: A Survey”, this paper mainly reviews knob tuning and only discuss index configuration, view configuration, partition configuration in section 6.3. However, index selection is an important research area studied for decades in database community and belongs to the configuration tuning category. To be fair and clear, this paper should be titled like “Automatic Database Knob Tuning: A Survey”.}
\end{Box4}

\vspace{-.5em}
\stitle{\bfit{Response:}} We have changed the title  to ``Automatic Database Knob Tuning: A Survey'', and made it consistent with the whole paper, \ie\ replacing $(i)$ ``configuration tuning'' with ``knob tuning'' and $(ii)$  ``configuration samples'' with ``knob setting samples''. %In addition, we also have made the other descriptions associated with the knobs consistent.


%Thank you for your suggestion. We have thoroughly analyzed the relevant papers published in SIGMDO/PVLDB/ICDE/TKDE, from which we find ``database tuning'' (16 out of 24 papers listed at https://github.com/evolveDB/tuning-survey) is most frequently used. Thus, we have renamed the paper as ``Automatic Database Tuning: A Survey''. And problems like index selection and view selection are classified into ``other database optimization problems''.

%We have renamed the paper to ``Automatic Database Knob Tuning: A Survey'', and made it consistent through the whole paper. \zxh{check by xinyang}


\begin{Box4}{}
    {\textbf{C2}: Unrealistic claim on BO-based and RL-based tuning methods and absence of the recent research observation on the two methods. %The survey claims “Traditional machine learning-based tuning methods rely on a large number of high-quality training data to learn the tuning knowledge. However, it is rather hard to obtain such training data. To address this limitation, reinforcement learning (RL) based methods have been proposed which explore promising configuration space with trial-and-error strategies without requiring prepared training data.” “Fourth, both BO-based methods and DL-based methods are based on supervised models, and they require a large number of training data, which may be costly to obtain or even unavailable in real scenarios. So RL-based methods are proposed to explore suitable knob settings based on the exploration-exploitation policies.” “Gaussian process cannot perform well for a large number of knobs or large-scale datasets, because it needs to explore huge configuration spaces. In addition, it also relies on high-quality historical configuration data, which is expensive to acquire”
    Both BO-based and RL-based tuning methods adopt trial-and-error manner to learn a promising configuration with exploration-exploitation policies. BO uses acquisition function balancing exploration-exploitation to guide the trial-and-errors. And BO are fundamentally used to sample limited points to maximize a black function.
    
And both BO-based and RL-based can collect samples during the model’s training without using historical data (learning from scratch). It actually depends on the settings of the developers. The justifications are unrealistic that the difficulty to collect training data or the relying on high-quality historical configuration data are the limitation of BO not the RL. Those claims the survey made lacks the insight on the RL and BO methods and should be removed.
}
\end{Box4}

\begin{Box4}{}
{
In addition, one recent experimental research [2] has shown the RL-based methods has inferior performance in limited tuning budget and more tuning overhead -- DDPG needs more iterations to learn the neural network than BO-based methods and more iterations to converge. The evaluation shows that ``DNN and GPR (BO-based) achieve 40\% better DB Time than the default configuration. DDPG and DDPG++ only achieve 18\% and 32\% improvement''. ``The optimized configuration for GPR (BO-based) achieves 27\% better DB Time than the SG default configuration. DNN performs the next best, improving the DB Time by 15\%. The configurations generated by DDPG++ and LHS improve the performance by less than 10\%. For DDPG, none of its optimized configurations that tune 20 knobs improved the DB Time over the default settings.'' ``This especially impacts DDPG and DDPG++ since they take longer to converge in general.''  And other studies [1][3][4] have the consistent observations. As a survey paper, those observation should be mentioned and the description should be objective.

[1] Black or White? How to Develop an AutoTuner for Memory-based Analytics [SIGMOD 2020]

[2] An Inquiry into Machine Learning-based Automatic Configuration Tuning Services on Real-World Database Management Systems [VLDB 2021]

[3] ResTune: Resource Oriented Tuning Boosted by Meta-Learning for Cloud Databases [SIGMOD 2021]

[4] Facilitating database tuning with hyper-parameter optimization: a comprehensive experimental evaluation [VLDB 2022].}
\end{Box4}

%\vspace{-.5em}
\stitle{\bfit{Response:}} Thank you for your insightful advice. First, we have removed the claim (\ie ``BO-based methods rely on high-quality historical data''). Specifically, both BO-based and RL-based methods can {\it start tuning without any historical data}. However, high-quality historical data can accelerate the tuning process of these methods. For example, both OtterTune~\cite{van2017automatic} (BO-based method) and WATuning~\cite{ge2021watuning} (RL-based method) utilize historical data to improve the tuning efficiency (see Section~\ref{sec:framework},~\ref{sec:methods}).

Second, we have clarified the pros and cons of BO-based and RL-based methods according to the (experimental) researches~\cite{van2021inquiry,DBLP:journals/pvldb/ZhangCLWTLC22,kanellis2022llamatune,kunjir2020black} in Section~\ref{sec:framework}. 

\lgl{should first summarize the pros/cons of BO and RL, and then give evidence from other papers. TOOOO fussy!!!!! --updated}

$\bullet$ {\it BO-based tuning methods} can efficiently find high-quality knob settings with the exploration-exploitation strategy and generally outperform heuristic methods~\cite{van2021inquiry,DBLP:journals/pvldb/ZhangCLWTLC22}. For the probability models adopted in BO-based tuning methods, $(i)$ Gaussian process is mainly suitable for continuous knobs, which can efficiently model different distributions and is most widely used in existing tuning methods; $(ii)$ SMAC can support both continuous and category knobs and scales better to many knobs than Gaussian process~\cite{DBLP:journals/pvldb/ZhangCLWTLC22}.


However, existing BO-based methods (especially those that adopt Gaussian process) are based on relatively simple probability distribution (\eg\ assuming the knob-performance relations following the Gaussian distribution) and may fall into sub-optimum for large configuration space. 

%Besides, for the surrogate models in BO-based tuning methods, $(i)$ the Gaussian process is mainly suitable for optimizing continuous knobs; $(ii)$ SMAC can support both continuous and category knobs and performs better than the Gaussian process for relatively large configuration space~\cite{DBLP:journals/pvldb/ZhangCLWTLC22}.

$\bullet$ {\it RL-based tuning methods} learn the tuning strategy by the interactions between the tuning model and target database, which are suitable for high-dimensional configuration space exploration. By allowing relatively sufficient tuning overhead (\eg\ 200 iterations in \cite{DBLP:journals/pvldb/ZhangCLWTLC22}), RL-based methods could outperform BO-based methods, which quickly converge but may stop at sub-optimal knob settings.


However, many scenarios strictly limit the tuning overhead, where RL-based methods may meet performance degradation. For example, in \cite{van2021inquiry}, within 150 iterations, RL-based methods could not fully optimize these knobs and perform worse than BO-based methods, because BO-based methods avoid approximating the complex metric-knob relationships and efficiently explore suitable knob settings.


%and updated the descriptions of BO-based and RL-based tuning methods as shown below: %and added the related papers~\cite{van2021inquiry,DBLP:journals/pvldb/ZhangCLWTLC22,kanellis2022llamatune} in Section~\ref{sec:methods}. 

%\lgl{do not use naive!!! the review mentioned that Bo can also use exploration-exploitation. why do you say that BO can only use random sampling? }%they begin the tuning process based on some configuration knob samples generated by sampling methods. 

%{\it Claim 1.:} Both BO-based methods and RL-based methods {\it use the exploration-exploitation policy in the tuning process}. BO-based methods use the surrogate model to map the knob-performance relationship. To initialize the surrogate model, they generally use sampling methods to generate some sample knob settings. BO-based methods use the acquisition function, which enables the balance between exploration and exploitation, to select some new knob settings. These new knob settings could be used to update the surrogate model. For RL-based methods, they use the interaction between the agent (tuning model) and the environment (database) to find knob settings.

%{\it Claim 2.:} Both BO-based methods and RL-based methods can {\it start tuning without any historical data}. However, high-quality historical training data could accelerate the tuning process for BO-based and RL-based methods. For example, OtterTune (a BO-based method in Section~\ref{subsec:gp}) and WATuning (an RL-based method in Section~\ref{subsec:drl}), use historical data to enhance the tuning procedure.

%\noindent $\bullet$ RL-based methods have two main advantages: (1) As discussed in many AI papers, traditional surrogate models in BO cannot efficiently support high-dimension space exploration~\cite{shahriari2015taking} and generally tunes a limited number of knobs. Although there are some attempts at high-dimension BO algorithms~\cite{kandasamy2015high,rolland2018high}, these algorithms have not been used in existing tuning works. Instead, RL-based methods can support more knobs with high-dimension space exploration~\cite{zhang2019end}; (2) Compared with BO-based methods, RL-based methods select knob settings based on both the past and (estimated) future selections \lgl{what is selection}, which help to avoid sub-optimum (verified in the experimental paper \cite{van2021inquiry}). \lgl{what results?}  \lgl{what is the effect of the second advantange?}


%\noindent $\bullet$ BO-based methods can quickly converge when tuning dozens of knobs. Instead, RL-based methods take a much longer time to learn the tuning strategy and recommend high-quality knob settings. Thus, it is hard for RL-based methods to converge within limited iterations (\eg requiring over 150 iterations).



%\noindent $\bullet$  \zxy{Both BO-based methods and RL-based methods use the exploration-exploitation policy in the tuning process. BO-based methods use the surrogate model to map the knob-performance relationship. To initialize the surrogate model, they generally use sampling methods to generate some sample knob settings. BO-based methods use the acquisition function, which enables the balance between exploration and exploitation, to select some new knob settings. These new knob settings could be used to update the surrogate model. For RL-based methods, they use the interaction between the agent (tuning model) and the environment (database) to find knob settings.}

%That is, BO-based methods generally initialize the tuning process by some observed knob settings~\cite{thummala2010ituned,kunjir2020black}; and RL-based methods try different knob settings with the exploration-exploitation mechanism.  

%\zxy{Both of these two methods can start tuning without any historical data. However, high-quality historical training data could accelerate the tuning process for BO-based and RL-based methods. For example, in OtterTune (a BO-based method illustrated in Section~\ref{subsec:gp}) and WATuning (an RL-based method illustrated in Section~\ref{subsec:drl}), use historical data to enhance the knob tuning.}

%can be utilized by both BO-based methods (model initialization) and RL-based methods (model pre-training), which avoid redundant model training (\eg reusing similar workloads) and enhance knob tuning.

%guide to the beneficial knob subspace and save unnecessary exploration time.


\iffalse
\hi{Empirical Tuning Findings.} Recently, some experimental papers~\cite{van2021inquiry,DBLP:journals/pvldb/ZhangCLWTLC22} have provided valuable empirical experience in which tuning methods are more suitable under different tuning scenarios (see Section~\ref{subsec:emprical-compare}). \lgl{why do you add this paragraph?} %We summarize the experience as follows.

\noindent $\bullet$ Aken et al.~\cite{van2021inquiry} separately tested heuristic/BO/DL/RL-based methods, where the learned models are trained for at most 150 iterations. And they find (1) heuristic methods (\eg LHS) are ineffective in exploring large knob space and perform worst; (2) RL-based methods and DL-based methods can find near-optimal knob settings for a few knobs (\eg 10 knobs selected by DBA), while BO-based methods may stop at sub-optimal knob settings; (3) BO-based methods converge quickly and could outperform RL-based methods when the knob number is large (\eg 40 knobs), because RL-based methods could not fully optimize these knobs within limited iterations. \lgl{you say RL is better for more knobs, but here BO outperforms RL. inconsistent!!!!!}

\noindent $\bullet$ Furthermore, Zhang et al.~\cite{DBLP:journals/pvldb/ZhangCLWTLC22} find (1) the metric-to-optimal-knob relations may not exist for a small number of knobs (\eg 5-20 knobs), \lgl{what is the connection of the two sentences?} where BO-based methods can achieve both better performance and lower overhead than RL-based methods, because BO-based methods can avoid approximating the complex relations and efficiently explore suitable knob settings; (2) In BO-based methods, the surrogate model SMAC scales better to relatively high knob space than other surrogate models (\eg Gaussian process, TPE), because SMAC can better learn the knob relations with the tree model (random forest); (3) With sufficient training (\eg 200 iterations), RL-based methods can find high-quality knobs in relatively large knob space, because the neural networks adopted in reinforcement learning have high configuration space representation capability.
\fi

%\noindent $\bullet$ Aken et al~\cite{van2021inquiry}: (1) They limit the tuning overhead as ``each method can run at most 150 iterations for each tuning scenario''; (2) Heuristic sampling methods (e.g., LHS) is inefficient for large knob space and perform worst; (3) DRL-based methods and DNN-based methods can find near-optimal knob settings for a small number of knobs (e.g., 10 knobs selected by DBA), while BO-based methods may stop at sub-optimal knob settings; (4) BO-based methods converge quickly under different numbers of knobs and may outperform the DRL-based methods for large number of knobs under strict iteration limits, where DRL-based methods could not fully optimize many knobs within limited iterations.

%\noindent $\bullet$ Zhang et al~\cite{DBLP:journals/pvldb/ZhangCLWTLC22}: (1) They extend the tuning overhead to 200 iterations; (2) BO-based methods can achieve better performance and lower overhead than DRL-based methods for relatively small knob space (e.g., 5-20 knobs), because the metric-to-optimal-knob relations (learned in DRL-based methods) may not exist for small knobs and BO-based methods can avoid approximating the complex relations and efficiently learn the knob setting distributions; (3) BO-based methods like SMAC (random-forest as surrogate model) scales better to relatively high knob space than other BO-based methods (e.g., gaussian process, TPE), because it can better learn the knob relations with the tree model; (4) DRL-based methods can find high-quality knobs in large knob space, because the neural networks used in DRL have high knob-space representation capability and require more iterations to update the network weights.

\iffalse
\begin{table}[]
\label{tab:my-table}
\begin{tabular}{|l|l|}
\hline
             & Observations                                                                                               \\ \hline
Relm~\cite{}         & \begin{tabular}[c]{@{}l@{}}1. RL-based methods (DDPG) need more iterations \\ to  converge than BO/DNN-based methods\end{tabular} \\ \hline
ResTune~\cite{}      &                                                                                                            \\ \hline
Aken et al.~\cite{}      &                                                                                                            \\ \hline
Zhang et al~\cite{} &                                                                                                            \\ \hline
\end{tabular}
\end{table}
\fi

%\vspace{-.5em}
\begin{Box4}{}
	{\textbf{C3}:  State the scenarios and metrics to analysis tuning methods.
		\\
		The paper lacks the clear statements on the scenarios and metrics used to analysis tuning methods and causes vague conclusions.
		For example, tuning performance (the performance of best configuration found), tuning overhead (the iteration needed to find good configuration), adaptability, safety are useful metrics to evaluate tuning methods. And in offline scenarios, tuning performance and tuning overhead are important. In online scenarios, safety and adaptability become more important.
	}
\end{Box4}

%\vspace{-.5em}
\stitle{\bfit{Response:}} Thank you for the insightful advice. We have clarified the statements on the four metrics and summarized their importance under different scenarios in Section~\ref{sec:introducion}.


%Recently many tuning works~\cite{van2017automatic,DBLP:journals/vldb/ZhangZLLXCX21, li2019qtune,zhang2019end,li2019qtune,van2021inquiry,DBBERT,DBLP:conf/sigmod/ZhangWCJT0Z021,DBLP:conf/sigmod/ZhangWCJT0Z021,DBLP:journals/pvldb/WangTB21,DBLP:journals/pvldb/ZhangCLWTLC22,DBLP:conf/sigmod/CaiLZZZLLCYX22,kunjir2020black,DBLP:conf/sigmod/ZhangW0T0022} have evaluated from the four metrics. We have comprehensively reviewed these papers and clarified the definition of the four metrics. 

\hi{Tuning Performance} aims to evaluate how well the method achieves the performance objectives (\eg latency and throughput~\cite{van2017automatic,DBLP:journals/vldb/ZhangZLLXCX21, li2019qtune}, resource usage~\cite{zhang2021restune,tan2019ibtune}) under the selected knob settings.

\hi{Tuning Overhead} aims to measure the consumed time or system resources for finding good knob settings~\cite{van2017automatic,van2021inquiry,li2019qtune} (added in Section~\ref{sec:introducion}). 

\hi{Tuning Adaptability.} According to \cite{van2021inquiry,zhang2019end,li2019qtune,DBLP:conf/sigmod/ZhangWCJT0Z021,DBLP:journals/pvldb/WangTB21,DBBERT,DBLP:journals/pvldb/ZhangCLWTLC22,DBLP:conf/sigmod/CaiLZZZLLCYX22}, we define {\it tuning adaptability} as the performance change after the tuning \zxh{scenario} has changed (\eg \ workload/hardware/db-version/db-system changes \lgl{enviorment?}). 

\noindent $\bullet$ Aken et al~\cite{van2021inquiry}: ``We train their models on one workload and then use them to tune another workload''. (workload)

\noindent $\bullet$ CDBTune~\cite{zhang2019end}: ``How to adapt to new environment (memory sizes) or workload changes''. (workload, hardware)

\noindent $\bullet$ QTune~\cite{li2019qtune}: ``The performance when workload or hardware (disk, RAM, CPU) changes''. (workload, hardware)

\noindent $\bullet$ ResTune~\cite{DBLP:conf/sigmod/ZhangWCJT0Z021}: ``Transfer between different hardware environments and varying workloads setting''. (workload, hardware)

\noindent $\bullet$ UDO~\cite{DBLP:journals/pvldb/WangTB21}: ``Vary the number of TPC-H queries; Shifting workload''. (dynamic workload)

\noindent $\bullet$ DB-BERT~\cite{DBBERT}: ``Avoid learning the names of specific parameters as they do not generalize across systems''. (systems)

\noindent $\bullet$ Zhang et al~\cite{DBLP:journals/pvldb/ZhangCLWTLC22}: ``Fine-tune its pre-trained model to adapt to the target workload''. (workload)

\noindent $\bullet$ Hunter~\cite{DBLP:conf/sigmod/CaiLZZZLLCYX22}: ``Read/write ratios change for online model reuse''. (workload)

For learning-based methods, tuning adaptability highly depends on the transfer capability of the well-trained tuning models (see R3C12). And the additional transfer techniques are explained in Section~\ref{subsec:transfer}.

\hi{Tuning Safety.} According to \cite{kunjir2020black,DBLP:conf/sigmod/ZhangW0T0022}, {\it tuning safety} is the capacity to select knob settings that will not cause significant performance degradation or even system crash.% (added in Section~\ref{subsec:gp}).

\noindent $\bullet$ RelM~\cite{kunjir2020black}: ``resource usage should be within allocation at all times''.

\noindent $\bullet$ OnlineTune~\cite{DBLP:conf/sigmod/ZhangW0T0022}: ``The tuner should recommend configurations that do not downgrade the database performance during the tuning process''.

\hi{Scenario Discussion.} As suggested by the reviewer, the above metrics have different importance in considering the tuning scenarios. %\zxh{not consistent with the main body}

Offline tuning methods mainly focus on tuning performance and overhead. These methods can take relatively long time to generate training data and update models. But they also have a threshold (\eg no longer than three days) to avoid too much resource waste if the model cannot converge. In this way, RL-based/DL-based methods are suitable to represent a huge knob space and explore near-optimal knob settings~\cite{DBLP:journals/pvldb/ZhangCLWTLC22,van2021inquiry}. 

Online tuning methods pay more attention to tuning adaptability (\eg handling various workloads or hardware settings) and safety (\eg avoiding performance regression). Since complex tuning models like RL may lead to bad actions, more efficient BO/heuristic-based methods~\cite{DBLP:conf/sigmod/ZhangW0T0022,zhu2017bestconfig} are generally adopted to conduct online tuning, which can start with a few initial samples and quickly converge at good knob settings.


%and their importance under different tuning scenarios. For example, for offline tuning, the performance is most important; while for online tuning, both adaptability and safety are critical. 

%Second, we have separately analyzed the existing tuning works from the four metrics and summarized the suitable tuning methods/methodologies under different scenarios.


%\noindent $\bullet$ For an offline tuning task, RL takes hours to days to find high-quality knob settings and can outperform all the other methods.

%\noindent $\bullet$ For an online tuning task, BO can quickly converge and recommend suitable knob settings, where RL may perform much worse (\zxh{xxx\%}) within a few iterations.

%\noindent $\bullet$ When transferring learned tuning models to new tasks, deep-learning-based method performs best, which can better generalize the learned knowledge on historical tasks than BO and is easier to converge than RL. Besides, there are some transferring techniques that help the origin BO/RL-based methods to better adapt to the new tasks.

\begin{Box4}{}
{\textbf{C4}: Remove the category, Learning-based Knob Selection.
		
The learning-based knob selection has blurred borders with the knob tuning methods and has never been discussed as a knob selection method except for the survey.
		
In addition, the survey states, “during knob tuning, we lower the possibility of selecting the unimportant knobs. To this end, reinforcement learning-based methods are proposed…They attempt to learn the interaction between the change of the knob values and the database performance. Based on the feedback of reward values, they can identify the most important knobs. Unimportant knobs are fed back with minor rewards at the initial iterations”}
\end{Box4}
\begin{Box4}{}
{
However, lower the possibility of selecting the unimportant knobs is commonalities of existing learning-based knob tuning methods, not a unique feature in RL. All the learning-based knob tuning methods tries to explore the promising area, varying the important knobs. It is unfair to state only RL learns the important knobs in section 1, section 3.2.3, table 3, etc.
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} We have removed the description of {\it learning-based knob selection} from Section~\ref{sec:knobs} and Table~\ref{tbl:knobselection} and clarified the common features (\eg\ identifying the important knobs during training) of learning-based methods in Section~\ref{sec:introducion}.

\begin{Box4}{}
	{\textbf{C5}:  In section 4.2.2, the paper states that selected metrics can be used “ to select important knobs, i.e., which metrics are sensitive to knob selection”. Please clearly state the relationship between knob selection and feature selection and how to use selected features to select important knobs.}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} 

\lgl{why only mention ottertune in these two paragraphs?}

Thank you for your valuable comments. We have clarified the relationship between feature selection and knob selection (Section~\ref{sec:framework},~\ref{sec:featureselection}). In \cite{van2017automatic,kanellis2020too}, they utilize the tuning objective metrics (\eg\ latency) to reflect the effects of different knobs to the database performance.

%In this survey, we divide the database metrics into database runtime metrics (in Section~\ref{subsec:workloads}) and performance metrics \ie latency and throughput (in Section~\ref{subsec:challenge}). Furthermore, the widely used metrics in current knob ranking modules are performance metrics (\eg latency or throughput)~\cite{van2017automatic, kanellis2020too}. Therefore, to avoid the confusion caused by the claim that ``selected metrics could be used to select important knobs, i.e., which metrics are sensitive to knob selection,'' we have removed this sentence and reorganized the description of database metrics.

%We have added the knob-feature relationship in Section~\ref{subsec:ranking}. Apart from representing the workload characteristics, the runtime metrics could also reflect the effects of knob settings on the database performance. For example, in OtterTune \cite{van2017automatic}, it indicates that if the knob controls the buffer pool size is low, then the metrics related to the number of buffer pool cache misses will increase. %Therefore, OtterTune uses the relevant metrics to select important knobs.  

%In Section \ref{subsec:ranking}, we have explained how OtterTune uses selected metrics to select important knobs, \ie taking knob settings samples as independent variables (X) and the selected metrics as dependent variables (y). It employs a regularized version of least squares to rank the knobs based on the effects on the metric value changes. %\zxh{what about other methods?}



\begin{Box4}{}
	{\textbf{C6}:  The analysis in section 5.2 Bayesian Optimization-based Tuning Methods should be improved.\\
		1. GP is only a surrogate model used in BO. And other surrogate can be adopted. For example, Tuneful adopts random forest instead of GP.
		\\
		“Basic Idea of GP”, “Key Modules in GP”, “GP model design” should be changed to “Basic Idea of BO”, “Key Modules in BO”,  “BO model design”.
		\\
		2. Key Modules in BO. Instead of Configuration Sample Initialization and G model, the key modules in BO are surrogate model and acquisition functions.
		\\
		3. Workload mapping is a transfer technique discussed in section Transfer Techniques, not limited in the initial initialization phase. It should not appear in section 5.2.
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} We have updated the analysis in Section~\ref{subsec:gp}. First, we have replaced the ``GP-based methods'' with ``BO-based methods'', where we separately introduced the core idea and four main modules in the BO-based methods, \ie\ surrogate model, acquisition functions, model initialization, and database features. In particular, most of the existing BO-based  methods~\cite{thummala2010ituned,van2017automatic,kunjir2020black,zhang2021restune,cereda2021cgptuner,DBLP:conf/sigmod/ZhangW0T0022} adopt Gaussian process as their surrogate model. And other surrogate models like SMAC and TPE are studied in \cite{DBLP:journals/pvldb/ZhangCLWTLC22,kanellis2022llamatune}. Second, as workload mapping is a transfer technique, we have moved the analysis of {\it workload mapping} methods from Section~\ref{subsec:gp} to Section~\ref{subsec:transfer}.



\begin{Box4}{}
	{\textbf{C7}: Missing citations and discussion about some knob tuning researches in database community.
		\\
		Facilitating database tuning with hyper-parameter optimization: a comprehensive experimental evaluation [VLDB 2022].
		\\
		LlamaTune: Sample-Efficient DBMS Configuration Tuning [VLDB 2022].
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} We have added these works~\cite{kanellis2022llamatune,DBLP:journals/pvldb/ZhangCLWTLC22}. 

% and accordingly updated Figure~\ref{fig:timeline1},~\ref{fig:gpworkflow} and Table~\ref{tbl:methodsummary}:

First, many BO-based methods assume that the values of each knob have equal importance at the beginning of knob tuning. However, this assumption may cause the special values in knobs (\eg\ in MySQL, the value 0 of {\it innodb\_thread\_concurrency} indicates no limitation of the supported parallel threads) to have lower probability of being selected than in real scenarios (frequently set as the default value). \lgl{the original paper used biased? --yes} Therefore, LlamaTune~\cite{kanellis2022llamatune} utilizes a biased sampling method, which sets a fixed probability for the special value of the knob,  to further explore the knob with special values in knob tuning. 

Second, \cite{DBLP:journals/pvldb/ZhangCLWTLC22} is an experimental paper. We have added some of the valuable findings in Section~\ref{sec:methods} (see R3C2). 



\begin{Box4}{}
	{\textbf{C8}: Definition 1 only considers continuous knobs and miss the categorial knobs which are quite common in DBMSs.}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} In Definition 1 (Section~\ref{subsec:knobs}), we have added the discussion of categorical knobs.

\begin{Box4}{}
	{\textbf{C9}:  Use clear terminologies about tuning overhead/ tuning cost.
		\\
		a. In table 1, there is a column name tuning cost for different knobs. And how to label the knobs as low, medium, high is not mentioned.
		\\
		b. In table 5, a column named tuning overhead for different methods.
		\\
		c. In figure 7, UDO is a tuning method that separates light/heavy knob tuning overhead.
		\\
		The tuning overhead has different contents and causes misunderstanding. It is better to refer to a and c as reconfiguration cost and clearly explain the terminologies.
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} First, {\it tuning cost} denotes the extra time for the new knob value to take effect (some knobs, like memory allocation, take a relatively long time). By following the reviewer's advice, we have renamed {\it tuning cost} to {\it reconfiguration cost} (involving Table~\ref{tbl:knobclasses}, Section~\ref{subsec:drl}, Figure~\ref{fig:rltree}) so as to distinguish it from tuning overhead (the time for a tuning method to find suitable knob values).

%\lgl{should use a better word. effection latency. let me think.}

\begin{Box4}{}
	{\textbf{C10}:  Inconsistent remark.
		\\
		Some sections use remark to summarize the pros and cons of related work while some sections not.
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} We have added remarks for each category of tuning methods in Section~\ref{sec:methods}.



\begin{Box4}{}
	{\textbf{C11}: The description of knobs can be improved. \\
		“For example, for query plan optimization, there are join collapse limit in Postgres, and rewrite enabled in MySQL; for cost values, there are seq page cost in Postgres and join buffer size in MySQL.” How do the knobs impact the query optimizers?
		\\
		“First, some knobs determine which physical operators can be utilized in the generated query plan.” Which knob, how to determine?
		\\
		In section 3.1.4, there should be some concrete knobs name and explanations.
		
	}
\end{Box4}

%\vspace{-.5em}

\stitle{\bfit{Response:}} First, we have added insights of the knob effects. For example, knobs like seq\_page\_cost can significantly affect the physical operator selection (e.g., lower seq\_page\_cost may cause the optimizer to select seq\_scan rather than index\_scan; lower random\_page\_cost may cause the optimizer to utilize indexes instead). 

Second, we have added concrete knob examples in Section~\ref{subsec:process}: ``In Postgres, for any sort operator whose input tuples are fewer than the value of {\it replacement\_sort\_tuples}, the database utilizes replacement-selection sort rather than quicksort to improve the sorting efficiency under limited memory. \lgl{which selection algorithm? hard to follow!!!}''; ``In MySQL, for high concurrency workloads, we can tune {\it innodb\_lock\_wait\_timeout} to control the waiting time for a lock before being rolled back''. \lgl{not a good example!!!! --updated}
% temporarily disable deadlock detection via {\it innodb\_deadlock\_detect} so as to ensure the execution efficiency; and 


\begin{Box4}{}
	{\textbf{C12}: In table 5, the column transfer capability needs declaration. Why only Manual and Heuristic (Search-based) has transfer capability?
	}
\end{Box4}
%\vspace{-.5em}

\stitle{\bfit{Response:}} Thank you for your advice. We have removed the ``transfer capability'' column in Table~\ref{tbl:methodsummary} and only discuss the transfer capability of learning-based tuning methods in Section~\ref{sec:methods}. First, many tuning methods characterize different database features so as to support workload/hardware/system changes.

$\bullet$ For workload changes, tuning methods characterize critical database features (\eg runtime metrics in OtterTune~\cite{van2017automatic}) or query features (\eg physical operators and costs in QTune~\cite{li2019qtune}, read/write ratios in WATuning~\cite{ge2021watuning}) and can efficiently adjust knob settings for new workloads. 


$\bullet$ For hardware changes, tuning methods like RelM~\cite{kunjir2020black} profile the underlying runtime characteristics (\eg shuffle memory usage, CPU usage for parallel tasks) and can generalize to different hardware requirements.

$\bullet$ For system changes, DB-BERT~\cite{DBBERT} trains a language model to extract common features (\eg numerical system characters) of knobs across systems. 

$\bullet$ Methods like ResTune~\cite{zhang2021restune} (common query features, model transferring) and CGPTuner~\cite{cereda2021cgptuner} (workload + IT features), OnlineTune~\cite{DBLP:conf/sigmod/ZhangW0T0022} (workload + data features) can adapt to both workload and underlying system changes.

Second, some tuning methods rely on transfer techniques to reuse historical samples/models, which are introduced in Section~\ref{subsec:transfer}.



%We have clearly defined ``transfer capability'', i.e., the tuning capability/availability on new scenarios. 
%Manual/heuristic methods own high transfer capability, because the human experience and algorithm do not need to update based on the workload/database characters. Instead, the origin learned models (BO-based and RL-based) have poor transfer capability, which are built based on the tuning characters, and take relatively long time to learn the new feature-knob-performance mapping relationships (without additional transferring techniques). Thus, the learned methods equipped with transferring techniques gain much higher transfer capability because they can reuse historical models to quickly build the suitable model in the new scenario.



\begin{Box4}{}
	{\textbf{C13}: grammatical and representation errors
		\\
		1. it can evaluate the quality of each search method and
		\\
		2. QTune uses a deep neural network…. QTune used a modified DDPG model…
		\\
		
	}
\end{Box4}


%\vspace{-.5em}

\stitle{\bfit{Response:}}  We have fixed these errors and carefully proofread the whole paper.

